Operational locality in global theories

Within a global physical theory, a notion of locality allows us to find and justify information-processing primitives, like non-signalling between distant agents. Here we propose exploring the opposite direction: to take agents as the basic building blocks through which we test a physical theory, and recover operational notions of locality from signalling conditions. First we introduce an operational model for the effective state spaces of individual agents, as well as the range of their actions. We then formulate natural secrecy conditions between agents and identify the aspects of locality relevant for signalling. We discuss the possibility of taking commutation of transformations as a primitive of physical theories, as well as applications to quantum theory and generalized probability frameworks. This "it from bit" approach establishes an operational connection between local action and local observations, and gives a global interpretation to concepts like discarding a subsystem or composing local functions.

==> tcbtheorems.code.tex <==
%% The LaTeX package tcolorbox - version 3.60 (2015/05/07)
%% tcbtheorems.code.tex: Code for theorems in colorboxes
%%
%% -------------------------------------------------------------------------------------------
%% Copyright (c) 2006-2014 by Prof. Dr. Dr. Thomas F. Sturm <thomas dot sturm at unibw dot de>
%% -------------------------------------------------------------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2005/12/01 or later.
%%
%% This work has the LPPL maintenance status `author-maintained'.
%%
%% This work consists of all files listed in README
%%
%\makeatletter
\tcb@set@library@version{3.60}

\RequirePackage{amsmath}

\def\tcb@hack@amsmath{\tcb@hack@currenvir\vskip-\abovedisplayskip}

\def\tcb@theo@form@namenumber#1#2{\hbox{#1~#2}}
\def\tcb@theo@form@numbername#1#2{\hbox{#2~#1}}
\def\tcb@theo@form@name#1#2{\hbox{#1}}

\def\tcb@theo@desc@form@std#1{\tcb@desc@col\kvtcb@desc@font\kvtcb@desc@delim@left#1\kvtcb@desc@delim@right}

\def\tcb@theo@title#1#2#3{%
  \ifdefempty{#2}{\setbox\z@=\color@hbox#1\color@endbox}{\setbox\z@=\tcb@theo@form{#1}{#2}}%
  \def\temp@a{#3}%
  \ifx\temp@a\@empty\relax%
    \unhbox\z@\kvtcb@terminatorsign%
  \else%
    \setbox\z@=\hbox{\unhbox\z@\kvtcb@separatorsign\ }%
    \hangindent\wd\z@%
    \hangafter=1%
    \mbox{\unhbox\z@}{\tcb@theo@desc@form{#3}}\kvtcb@terminatorsign%
  \fi%
}

\def\tcb@theo@listentry#1#2#3{%
  \def\kvtcb@listentry{\protect\numberline{#2}#3}%
}

\def\tcb@theo@label#1#2{%
  \def\temp@a{#2}%
  \ifx\temp@a\@empty%
  \else%
    \tcbset{label={#1:#2}}%
  \fi%
}

\if@fleqn%
\tcbset{%
  ams equation upper/.style={before upper=\tcb@hack@amsmath\equation,after upper=\endequation},%
  ams equation lower/.style={before lower=\tcb@hack@amsmath\equation,after lower=\endequation},%
  ams equation* upper/.style={before upper=\tcb@hack@amsmath\csname equation*\endcsname,after upper=\endequation},%
  ams equation* lower/.style={before lower=\tcb@hack@amsmath\csname equation*\endcsname,after lower=\endequation}%
}%
\else%
\tcbset{%
  ams equation upper/.style={before upper=\tcb@hack@currenvir\equation,after upper=\endequation},%
  ams equation lower/.style={before lower=\tcb@hack@currenvir\equation,after lower=\endequation},%
  ams equation* upper/.style={before upper=\tcb@hack@currenvir\csname equation*\endcsname,after upper=\endequation},%
  ams equation* lower/.style={before lower=\tcb@hack@currenvir\csname equation*\endcsname,after lower=\endequation},%
}%
\fi

\tcbset{
  theorem/.style args={#1#2#3#4}{%
    step and label={#2}{#4},%
    title={\letcs\tcb@temp{the#2}\tcb@theo@title{#1}{\tcb@temp}{#3}}},%
  math upper/.style={before upper=$\displaystyle,after upper=$},%
  math lower/.style={before lower=$\displaystyle,after lower=$},%
  math/.style={math upper,math lower},%
  ams equation/.style={ams equation upper,ams equation lower},%
  ams equation*/.style={ams equation* upper,ams equation* lower},%
  ams align upper/.style={before upper=\tcb@hack@amsmath\align,after upper=\endalign},%
  ams align lower/.style={before lower=\tcb@hack@amsmath\align,after lower=\endalign},%
  ams align/.style={ams align upper,ams align lower},%
  ams align* upper/.style={before upper=\tcb@hack@amsmath\csname align*\endcsname,after upper=\endalign},%
  ams align* lower/.style={before lower=\tcb@hack@amsmath\csname align*\endcsname,after lower=\endalign},%
  ams align*/.style={ams align* upper,ams align* lower},%
  ams gather upper/.style={before upper=\tcb@hack@amsmath\gather,after upper=\endgather},%
  ams gather lower/.style={before lower=\tcb@hack@amsmath\gather,after lower=\endgather},%
  ams gather/.style={ams gather upper,ams gather lower},%
  ams gather* upper/.style={before upper=\tcb@hack@amsmath\csname gather*\endcsname,after upper=\endgather},%
  ams gather* lower/.style={before lower=\tcb@hack@amsmath\csname gather*\endcsname,after lower=\endgather},%
  ams gather*/.style={ams gather* upper,ams gather* lower},%
  ams nodisplayskip upper/.style={before upper=\vskip-\abovedisplayskip},%
  ams nodisplayskip lower/.style={before lower=\vskip-\abovedisplayskip},%
  ams nodisplayskip/.style={ams nodisplayskip upper,ams nodisplayskip lower},%
  highlight math style/.style={highlight math/.style={notitle,nophantom,#1}},%
  separator sign/.store in=\kvtcb@separatorsign,%
  separator sign colon/.style={separator sign={:}},%
  separator sign dash/.style={separator sign={\ --}},%
  separator sign none/.style={separator sign=},%
  terminator sign/.store in=\kvtcb@terminatorsign,%
  terminator sign colon/.style={terminator sign={:}},%
  terminator sign dash/.style={terminator sign={\ --}},%
  terminator sign none/.style={terminator sign=},%
  description delimiters/.code 2 args={\def\kvtcb@desc@delim@left{#1}\def\kvtcb@desc@delim@right{#2}},%
  description delimiters parenthesis/.style={description delimiters=()},
  description delimiters none/.style={description delimiters={}{}},
  description color/.code={\def\temp@a{#1}\ifx\temp@a\@empty\relax%
    \def\tcb@desc@col{}\else\def\tcb@desc@col{\color{#1}}\fi},%
  description color/.default=,
  description font/.store in=\kvtcb@desc@font,
  description font/.default=,
  description formatter/.code={\let\tcb@theo@desc@form=#1},%
  description formatter/.default={\tcb@theo@desc@form@std},%
  theorem name and number/.code={\let\tcb@theo@form=\tcb@theo@form@namenumber},
  theorem number and name/.code={\let\tcb@theo@form=\tcb@theo@form@numbername},
  theorem name/.code={\let\tcb@theo@form=\tcb@theo@form@name},
  theorem style/.is choice,
  theorem style/standard/.style={separator sign colon,description delimiters none,
    terminator sign none,theorem name and number,attach title},
  theorem style/change standard/.style={theorem style=standard,theorem number and name},
  theorem style/plain/.style={separator sign none,description delimiters parenthesis,
    terminator sign colon,theorem name and number,attach title to upper={\ }},
  theorem style/plain apart/.style={separator sign none,description delimiters parenthesis,
    terminator sign none,theorem name and number,attach title},
  theorem style/break/.style={theorem style=plain,attach title to upper={\par}},
  theorem style/change/.style={theorem style=plain,theorem number and name},
  theorem style/change apart/.style={theorem style=plain apart,theorem number and name},
  theorem style/change break/.style={theorem style=break,theorem number and name},
  theorem style/margin/.style={theorem style=plain,theorem name,before title=\makebox[0pt][r]{\thetcbcounter\ }},
  theorem style/margin apart/.style={theorem style=margin,attach title,terminator sign none},
  theorem style/margin break/.style={theorem style=margin,attach title to upper={\par}},
}

\newcommand{\new@tcbtheorem}[5][]{%
  \@@newtcolorbox[auto counter,#1]{#2}[3][]{#4,%
    title={\tcb@theo@title{#3}{\thetcbcounter}{##2}},%
    list entry={\protect\numberline{\thetcbcounter}##2},%
    code={\tcb@theo@label{#5}{##3}},%
    ##1}%
  \@@newtcolorbox[#1,no counter,list inside=]{#2*}[2][]{#4,%
    title={\tcb@theo@title{#3}{\@empty}{##2}},%
    ##1}%
}

\def\newtcbtheorem{\let\@@newtcolorbox\newtcolorbox%
  \new@tcbtheorem}

\def\renewtcbtheorem{\let\@@newtcolorbox\renewtcolorbox%
  \new@tcbtheorem}

\newcommand{\tcbmaketheorem}[5]{%
  \newtcolorbox{#1}[3][]{#3,theorem={#2}{#4}{##2}{#5:##3},##1}%
}

\newtcbox{\tcboxmath}[1][]{nobeforeafter,math upper,tcbox raise base,#1}
\newtcbox{\tcbhighmath}[1][]{highlight math,nobeforeafter,math upper,tcbox raise base,#1}

\tcbset{%
  reset@theorems/.style={%
    description formatter,description color,description font,
    highlight math style={colframe=red,colback=yellow!25!white},%
    theorem style=standard,%
  },
  initialize@reset=reset@theorems,
}


